On the convergence of residual distribution schemes for the compressible Euler equations via dissipative weak solutions

In this work, we prove the convergence of residual distribution schemes to dissipative weak solutions of the Euler equations. We need to guarantee that the residual distribution schemes are fulfilling the underlying structure preserving properties such as positivity of density and internal energy. Consequently, the residual distribution schemes lead to a consistent and stable approximation of the Euler equations. Our result can be seen as a generalization of the Lax-Richtmyer equivalence theorem to nonlinear problems that consistency plus stability is equivalent to convergence.

==> Lipchitz.tex <==
\newpage

For the residual $\Phi_\sigma^K(\CU^h)$, we define its stencil $\mathcal{S}_\sigma$ the set of degrees of freedom that are needed to evaluate it, in other words,
$$\Phi_\sigma^K(\CU^h)=\Phi_\sigma^K(\CU_{\sigma'}, \sigma'\in \mathcal{S}_\sigma.$$
The following assumption is made on the residual:

 \begin{assumption}
\label{H2} Let $\TT_h$ be a triangulation satisfying the assumption \ref{H0}.
For any $C\in \R^+$, there exists $C'( C, \TT_h)\in \R^+$ which depends only on 
$C$ and $\TT_h$ such that for any 
$ \bU \in V^h, \text{ with } \norm{\bU}_{L^{\infty}(\R^2)}\leq C$ we have 
\begin{equation}
\label{eq:conservation}
\forall K, \forall \sigma, \norm{\Phi_{\sigma}^{K}}\leq C'(C, \TT_h) \; h\;
\sum_{\sigma'\in \mathcal{S}_\sigma}\norm{\bU_{\sigma'}-\bU_{\sigma}}.
\end{equation}
\end{assumption}

\newpage

==> assumption.tex <==
\newpage

\paragraph{Evaluation of the error}

\subsubsection*{Consistency Errors}
First, we realize that  for all $\varphi \in C^{p+1}( [0,T]\otimes \overline{\Omega}, \R^4)$
\begin{equation}\label{eq_consistent_2}
  \left[\int_{\Omega} \CU^h  \varphi\diff \bx \right]_{t=0}^{t=\tau}
  = \int_0^\tau \int_{\Omega} \frac{\diff{} }{\diff t} \left( \CU^h \varphi\right)\diff \bx \diff t 
  = \int_0^\tau \int_{\Omega} \CU^h \partial_t \varphi +  \varphi \partial_t \CU^h   \diff \bx\diff t
\end{equation}
and for the last term, we have to   apply the RD scheme in the semidiscrete setting \eqref{semi_unsteady}  for $\partial_t \CU^h$.
\newpage
